Optimal Solutions for Joint Beamforming and Antenna Selection: From Branch and Bound to Graph Neural Imitation Learning

This work revisits the joint beamforming (BF) and antenna selection (AS) problem, as well as its robust beamforming (RBF) version under imperfect channel state information (CSI). Such problems arise due to various reasons, e.g., the costly nature of the radio frequency (RF) chains and energy/resource-saving considerations. The joint (R)BF\&AS problem is a mixed integer and nonlinear program, and thus finding {\it optimal solutions} is often costly, if not outright impossible. The vast majority of the prior works tackled these problems using techniques such as continuous approximations, greedy methods, and supervised machine learning -- yet these approaches do not ensure optimality or even feasibility of the solutions. The main contribution of this work is threefold. First, an effective {\it branch and bound} (B\&B) framework for solving the problems of interest is proposed. Leveraging existing BF and RBF solvers, it is shown that the B\&B framework guarantees global optimality of the considered problems. Second, to expedite the potentially costly B\&B algorithm, a machine learning (ML)-based scheme is proposed to help skip intermediate states of the B\&B search tree. The learning model features a {\it graph neural network} (GNN)-based design that is resilient to a commonly encountered challenge in wireless communications, namely, the change of problem size (e.g., the number of users) across the training and test stages. Third, comprehensive performance characterizations are presented, showing that the GNN-based method retains the global optimality of B\&B with provably reduced complexity, under reasonable conditions. Numerical simulations also show that the ML-based acceleration can often achieve an order-of-magnitude speedup relative to B\&B.

==> tex/literature_ref.tex <==
sanaysanayei2004antenna: Antenna Selection in MIMO Systems
    Talks about RX/TX antenna selection. 
    Mentions that limited RF chain is the cause
    
Joint Power and Antenna Selection Optimization in Large Cloud Radio Access Networks 
An Liu, Member, IEEE, and Vincent K. N. Lau, Fellow, IEEE
 - Antenna selection to expensive CSI acqui- sition and signal processing overheads
 
Active Antenna Selection in Multiuser MIMO Communications, 2007
Mirette Sadek, Student Member, IEEE, Alireza Tarighat, Member, IEEE, and Ali H. Sayed, Fellow, IEEE 
 - Zero forcing requires the sum total of receive antennas to be less than that of the transmit antennas. 
 - This can be ensured by shutting down users or receive antennas judiciously 
 
Capacity of MIMO Systems With Antenna Selection, 2005
Andreas F. Molisch, Fellow, IEEE, Moe Z. Win, Fellow, IEEE, Yang-Seok Choi, Member, IEEE, and Jack H. Winters, Fellow, IEEE
    - Reduce the MIMO complexity
    - When receive antennas is larger than transmit, additional antennas do not provide noticeable gain. 
    - Focus on selection diversity
    
Antenna Selection for Energy-Efficient MIMO Transmission, 2012
Chenzi Jiang, Student Member, IEEE, and Leonard J. Cimini, Fellow, IEEE
    - Antenna selection that maximizes energy efficiency (bits per joule of energy)
    
    
A Fast And Optimal Deterministic Algorithm For NP-Hard Antenna Selection Problem
    Naveed Iqbal, Christian Schneider and Reiner S. Thom ̈a
    - Reference about NP hardness of the transmit antenna selection problem
